Transformer Neural Processes: Uncertainty-Aware Meta Learning Via Sequence Modeling

Neural Processes (NPs) are a popular class of approaches for meta-learning. Similar to Gaussian Processes (GPs), NPs define distributions over functions and can estimate uncertainty in their predictions. However, unlike GPs, NPs and their variants suffer from underfitting and often have intractable likelihoods, which limit their applications in sequential decision making. We propose Transformer Neural Processes (TNPs), a new member of the NP family that casts uncertainty-aware meta learning as a sequence modeling problem. We learn TNPs via an autoregressive likelihood-based objective and instantiate it with a novel transformer-based architecture. The model architecture respects the inductive biases inherent to the problem structure, such as invariance to the observed data points and equivariance to the unobserved points. We further investigate knobs within the TNP framework that tradeoff expressivity of the decoding distribution with extra computation. Empirically, we show that TNPs achieve state-of-the-art performance on various benchmark problems, outperforming all previous NP variants on meta regression, image completion, contextual multi-armed bandits, and Bayesian optimization.

==> figures/TNPs_backup.tex <==

% NEURAL NETWORK with coefficients, no arrows
\begin{figure*}
\centering
\begin{tikzpicture}[scale=0.6, every node/.style={scale=0.6}]

\def\xa{1.5}
\def\ya{0}
\def\xb{\xa+5.5}
\def\xc{\xb+5.25}
\def\yb{\ya+5.25}

\node[node 1, minimum size=50] (xy_1) at (\xa+0, \ya) {$x_1, y_1$};
\node[rectangle, draw, rounded corners, minimum width=1.7cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embxy_1) at (\xa+0, \ya+1.65){};

\filldraw[black] (\xa+1.25,\ya) circle (1pt);
\filldraw[black] (\xa+1.5,\ya) circle (1pt);
\filldraw[black] (\xa+1.75,\ya) circle (1pt);

\node[node 1, minimum size=50] (xy_m) at (\xa+3, \ya) {$x_m, y_m$};
\node[rectangle, draw, rounded corners, minimum width=1.7cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embxy_m) at (\xa+3, \ya+1.65){};

\node[node 1,fill=mygreen!5,draw=mygreen!20, minimum size=50] (xy_m+1) at (\xa+5.25, \ya) {$x_{m+1}, y_{m+1}$};
\node[rectangle, draw, rounded corners, minimum width=1.7cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embxy_m+1) at (\xa+5.25, \ya+1.65){};

\filldraw[black] (\xb+1,\ya) circle (1pt);
\filldraw[black] (\xb+1.25,\ya) circle (1pt);
\filldraw[black] (\xb+1.5,\ya) circle (1pt);

\node[node 1,fill=mygreen!5,draw=mygreen!20, minimum size=50] (xy_N) at (\xb+2.75, \ya) {$x_N, y_N$};
\node[rectangle, draw, rounded corners, minimum width=1.7cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embxy_N) at (\xb+2.75, \ya+1.65){};

\node[node 3, minimum size=50] (x_m+1) at (\xb+5, \ya) {$x_{m+1}, 0$};
\node[rectangle, draw, rounded corners, minimum width=1.7cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embx_m+1) at (\xb+5, \ya+1.65){};

\filldraw[black] (\xc+1,\ya) circle (1pt);
\filldraw[black] (\xc+1.25,\ya) circle (1pt);
\filldraw[black] (\xc+1.5,\ya) circle (1pt);

\node[node 3, minimum size=50] (x_N) at (\xc+2.75, \ya) {$x_N, 0$};
\node[rectangle, draw, rounded corners, minimum width=1.7cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embx_N) at (\xc+2.75, \ya+1.65){};

\node[node 3, minimum size=50] (ym+1_p) at (\xb+5, \yb) {$\hat{y}_{m+1}$};
\node[node 3, minimum size=50] (yN_p) at (\xc+2.75, \yb) {$\hat{y}_N$};

\filldraw[black] (\xc+1,\yb) circle (1pt);
\filldraw[black] (\xc+1.25,\yb) circle (1pt);
\filldraw[black] (\xc+1.5,\yb) circle (1pt);

\node[rectangle, draw,rounded corners, minimum width=15.25cm,minimum height=1.25cm, fill=myblue!20, align=center] (tr) at (\xb+1.25, \ya+3.15){Masked Self-attention};

\draw [->] (xy_1) to  (xy_1 |- embxy_1.south);
\draw [->] (xy_m) to  (xy_m |- embxy_m.south);
\draw [->] (xy_m+1) to  (xy_m+1 |- embxy_m+1.south);
\draw [->] (xy_N) to  (xy_N |- embxy_N.south);
\draw [->] (x_m+1) to  (x_m+1 |- embx_m+1.south);
\draw [->] (x_N) to  (x_N |- embx_N.south);

\draw [->] (embxy_1) to (embxy_1 |- tr.south);
\draw [->] (embxy_m) to (embxy_m |- tr.south);
\draw [->] (embxy_m+1) to (embxy_m+1 |- tr.south);
\draw [->] (embxy_N) to (embxy_N |- tr.south);
\draw [->] (embx_m+1) to (embx_m+1 |- tr.south);
\draw [->] (embx_N) to (embx_N |- tr.south);

\draw [<-] (ym+1_p) to (ym+1_p |- tr.north);
\draw [<-] (yN_p) to (yN_p |- tr.north);

\end{tikzpicture}
\caption{The general architecture of TNPs. For TNP-D and TNP-ND, the input sequence does not contain $\{(x_i, y_i)_{i=m+1}^N\}$.
% \ag{not sure if it is cleaner, but would the masking (i.e, fewer of the previous tokens would need to be masked i believe) be more efficient if we depict $(x,0)_j$ alongside $(x,y)_j$ for $j>m$?}
% \tu{I was thinking about doing that too. However I prefer the current ordering of tokens for 2 reasons: 1) it splits the input sequence into 3 sub-sequences, which aligns with how we present the masking mechanism in Section 4.1; 2) it positions $(x,y)_{j>m}$ next to each other, thus we can fade them to imply that they are not always required}
}
\label{fig:TNP_general}
\end{figure*}

==> figures/sequence_modeling.tex <==

% NEURAL NETWORK with coefficients, no arrows
\begin{figure}
\centering
% \begin{subfigure}[b]{\textwidth}
% \centering
\begin{tikzpicture}[scale=0.57, every node/.style={scale=0.57}]
% [x=2.2cm,y=1.4cm]

\def\xa{1.5}
\def\ya{0}
\def\xb{\xa+4}
\def\xc{\xb+7.5}
\def\yb{\ya+2.5}
\def\yc{\yb+1.5}

\node[node 1, minimum size=28] (x_1) at (\xa+0, \ya) {$x_1$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embx_1) at (\xa+0, \ya+1.25){};
\node[node 3, minimum size=28] (y_1) at (\xa+1.5, \ya) {$y_1$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (emby_1) at (\xa+1.5, \ya+1.25){};
\node[rectangle, draw, dashed, rounded corners, minimum width=2.75cm,minimum height=1.25cm] (box_1) at (\xa+0.75, \ya){};

\filldraw[black] (\xa+2.5,\ya) circle (1pt);
\filldraw[black] (\xa+2.75,\ya) circle (1pt);
\filldraw[black] (\xa+3,\ya) circle (1pt);

\node[node 1, minimum size=28] (x_m) at (\xb+0, \ya) {$x_m$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embx_m) at (\xb+0, \ya+1.25){};
\node[node 3, minimum size=28] (y_m) at (\xb+1.5, \ya) {$y_m$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (emby_m) at (\xb+1.5, \ya+1.25){};
\node[rectangle, draw, dashed, rounded corners, minimum width=2.75cm,minimum height=1.25cm] (box_m) at (\xb+0.75, \ya){};

\node[node 1, minimum size=28] (x_m+1) at (\xb+3.5, \ya) {$x_{m+1}$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embx_m+1) at (\xb+3.5, \ya+1.25){};
\node[node 3, minimum size=28] (y_m+1) at (\xb+5, \ya) {$y_{m+1}$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (emby_m+1) at (\xb+5, \ya+1.25){};
\node[rectangle, draw, dashed, rounded corners, minimum width=2.75cm,minimum height=1.25cm] (box_m+1) at (\xb+4.25, \ya){};

\filldraw[black] (\xb+6,\ya) circle (1pt);
\filldraw[black] (\xb+6.25,\ya) circle (1pt);
\filldraw[black] (\xb+6.5,\ya) circle (1pt);

\node[node 1, minimum size=28] (x_N) at (\xc+0, \ya) {$x_N$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (embx_N) at (\xc+0, \ya+1.25){};
\node[node 3, minimum size=28] (y_N) at (\xc+1.5, \ya) {$y_N$};
\node[rectangle, draw, rounded corners, minimum width=1cm,minimum height=0.5cm, fill=myyellow!50, align=center] (emby_N) at (\xc+1.5, \ya+1.25){};
\node[rectangle, draw, dashed, rounded corners, minimum width=2.75cm,minimum height=1.25cm] (box_N) at (\xc+0.75, \ya){};

\node[rectangle, draw,rounded corners, minimum width=14.25cm,minimum height=1.0cm, fill=myblue!20, align=center] (tr) at (\xb+2.5, \yb){Autoregressive Sequence Modeling};

\node[node 3, minimum size=28] (yhat_m+1) at (\xb+3.5, \yc) {$\hat{y}_{m+1}$};
\filldraw[black] (\xb+5,\yc) circle (1pt);
\filldraw[black] (\xb+5.5,\yc) circle (1pt);
\filldraw[black] (\xb+6,\yc) circle (1pt);
\node[node 3, minimum size=28] (yhat_N) at (\xc+0, \yc) {$\hat{y}_{N}$};

\draw [->] (x_1) to  (embx_1 |- embx_1.south);
\draw [->] (y_1) to  (emby_1 |- emby_1.south);
\draw [->] (x_m) to  (embx_m |- embx_m.south);
\draw [->] (y_m) to  (emby_m |- emby_m.south);
\draw [->] (x_m+1) to  (embx_m+1 |- embx_m+1.south);
\draw [->] (y_m+1) to  (emby_m+1 |- emby_m+1.south);
\draw [->] (x_N) to  (embx_N |- embx_N.south);
\draw [->] (y_N) to  (emby_N |- emby_N.south);

\draw [->] (embx_1) to  (embx_1 |- tr.south);
\draw [->] (emby_1) to  (emby_1 |- tr.south);
\draw [->] (embx_m) to  (embx_m |- tr.south);
\draw [->] (emby_m) to  (emby_m |- tr.south);
\draw [->] (embx_m+1) to  (embx_m+1 |- tr.south);
\draw [->] (emby_m+1) to  (emby_m+1 |- tr.south);
\draw [->] (embx_N) to  (embx_N |- tr.south);
\draw [->] (emby_N) to  (emby_N |- tr.south);

\draw [<-] (yhat_m+1) to (yhat_m+1 |- tr.north);
\draw [<-] (yhat_N) to (yhat_N |- tr.north);

% \draw [->] (xy_1) to  (xy_1 |- tr.south);
% \draw [->] (xy_m) to  (xy_m |- tr.south);
% \draw [->] (xy_m+1) to  (xy_m+1 |- tr.south);
% \draw [->] (xy_N) to  (xy_N |- tr.south);
% \draw [->] (x_m+1) to  (x_m+1 |- tr.south);
% \draw [->] (x_N) to  (x_N |- tr.south);

% \draw [<-] (ym+1_p) to (ym+1_p |- tr.north);
% \draw [<-] (yN_p) to (yN_p |- tr.north);

\end{tikzpicture}

\caption{Meta learning as sequence modeling. The sequence model autoregressively predicts the target given the context.}
\label{fig:sequence_modeling}
\end{figure}
